Maestro: A 302 GFLOPS/W and 19.8GFLOPS RISC-V Vector-Tensor Architecture for Wearable Ultrasound Edge Computing

Most Wearable Ultrasound (WUS) devices lack the computational power to process signals at the edge, instead relying on remote offload, which introduces latency, high power consumption, and privacy concerns. We present Maestro, a RISC-V SoC with unified Vector-Tensor Unit (VTU) and memory-coupled Fast Fourier Transform (FFT) accelerators targeting edge processing for wearable ultrasound devices, fabricated using low-cost TSMC 65nm CMOS technology. The VTU achieves peak 302GFLOPS/W and 19.8GFLOPS at FP16, while the multi-precision 16/32-bit floating-point FFT accelerator delivers peak 60.6GFLOPS/W and 3.6GFLOPS at FP16, We evaluate Maestro on a US-based gesture recognition task, achieving 1.62GFLOPS in signal processing at 26.68GFLOPS/W, and 19.52GFLOPS in Convolutional Neural Network (CNN) workloads at 298.03GFLOPS/W. Compared to a state-of-the-art SoC with a similar mission profile, Maestro achieves a 5x speedup while consuming only 12mW, with an energy consumption of 2.5mJ in a wearable US channel preprocessing and ML-based postprocessing pipeline.

==> Authors/Authors_bio_no_picture.tex <==
\begin{IEEEbiographynophoto}{Mattia Sinigaglia} received his Master’s Degree in Electronic Engineering from the University of Bologna in July 2021. He is currently pursuing a Ph. D. in Digital Systems Design at the Department of Electrical and Information Engineering (DEI) of the University of Bologna.  His research interest is semiconductor engineering for ultra-low-power devices, mainly targeting hardware-software co-design of RISC-V-based heterogeneous System-on-Chip.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Marco Bertuletti}
received the B.Sc. and M.Sc. degree in Electrical Engineering in Politecnico di Milano, Milano, Italy. He is currently pursuing his Ph.D. at ETH, Zurich, Switzerland, in the Integrated Systems Laboratory (IIS). His main interests are in the design of multi and many-core clusters of RISC-V processors for next-generation telecommunications.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Amirhossein Kiamarzi} received his Master’s degree in Computer Engineering from the University of Shiraz in 2020. He is currently pursuing a Ph.D. in Digital Systems Design at the Department of Electrical and Information Engineering (DEI), University of Bologna. His research focuses on modeling RISC-V-based hardware cores and accelerators.

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Luigi Ghionda} received his Master’s Degree in Electronic Engineering in March 2024 from the University of Bologna. He is currently a reaserch fellow in the group of Professor Luca Benini at the Department of Electrical and Information Engineering (DEI) of the University of Bologna. His research interests include the design of PULP (Parallel Ultra-Low Power)-based hardware accelerators and the design of RISC-V-based computer architectures for space SoC. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Riccardo Tedeschi} earned his Master’s Degree in Electronic Engineering from the University of Bologna in 2023. He is currently a Ph.D. candidate in Digital Systems Design at the Department of Electrical and Information Engineering (DEI) at the University of Bologna. His research focuses on RISC-V architectures for high-performance embedded platforms, with an emphasis on performance and reliability.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Aurora Di Giampietro} received her Master’s Degree in Electronic Engineering in February 2024 from the University of Bologna. She is currently working as a Research and Development Engineer at Onsemi in Switzerland. Her research interests focus on designing and developing low-power ASICs, with a particular emphasis on energy-efficient solutions for advanced electronic systems.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Mattia Orlandi} received his M.Sc. degree in Artificial Intelligence from the University of Bologna, Italy, in 2022. He is currently working toward his Ph.D. in Data Science and Computation under the supervision of Prof. S. Benatti at the Energy-Efficient Embedded Systems Laboratory (EEES Lab), DEI Department, University of Bologna. His research activities involve bio-signal processing with machine learning on low-power computing platforms. He is investigating how to decode EMG signals into spike trains to develop advanced human-machine interfaces.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Simone Benatti} received the Ph.D. degree in electrical engineering and computer science from the University of Bologna, Bologna, Italy, in 2016. He has collaborated with several international research institutes and companies. Previously, he worked for 8 years as an Electronic Designer and R\&D Engineer of electromedical devices. He has authored or coauthored more than 50 papers in international peer-reviewed conferences and journals. His research interests focus on energy efﬁcient embedded wearable systems, signal processing, sensor fusion, and actuation systems. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Yvan Tortorella} received his Master’s Degree in Electronic Engineering in October 2021 from the University of Bologna. He is currently pursuing a Ph. D. in Digital Systems Design in the group of Professor Luca Benini at the Department of Electrical and Information Engineering (DEI) of the University of Bologna. His research interests include the design of PULP (Parallel Ultra-Low Power)-based hardware accelerators for ultra-low power Machine Learning and the design of RISC-V-based computer architectures for satellite applications. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Luca Bertaccini} 
received his Ph.D. degree in Electrical Engineering from ETH Zurich in 2025, where he is currently a postdoctoral researcher in the Digital Circuits and Systems Group of Prof. Benini. His research interests include energy-efficient hardware accelerators, computer arithmetic, and heterogeneous systems-on-chip.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Giuseppe Tagliavini} is a Tenure-Track Assistant Professor at the University of Bologna. His research interests are focused on programming models, orchestration tools, and compiler optimizations for AI-enabled resource-constrained computing platforms, with a strong emphasis on parallel architectures and accelerators in the context of ultra-low-power IoT end nodes. He is a member of the IEEE and ACM societies.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Luca Benini} holds the chair of digital Circuits and systems at ETHZ and is Full Professor at the Universit\`{a} di Bologna. He received a PhD from Stanford University. Dr. Benini’s research interests are in energy-efficient parallel computing systems, smart sensing micro-systems and machine learning hardware. He has published more than 1000 peer-reviewed papers and five books. He is a Fellow of the ACM and a member of the Academia Europaea.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Francesco Conti} 
received the Ph.D. degree in electronic engineering from the University of Bologna, Italy, in 2016. He is currently a Tenure-Track Assistant Professor with the DEI Department, University of Bologna. From 2016 to 2020, he held a research grant with the University of Bologna and a Post-Doctoral Researcher with ETH Zürich. His research is centered on hardware acceleration in ultra-low power and highly energy efficient platforms, with a particular focus on System-on-Chips for Artificial Intelligence applications. His research work has resulted in more than 70 publications in international conferences and journals and was awarded several times, including the 2020 IEEE TCAS-I Darlington Best Paper Award
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Davide Rossi} received the Ph.D. degree from the University of Bologna, Bologna, Italy, in 2012. He has been a Post-Doctoral Researcher with the Department of Electrical, Electronic and Information Engineering “Guglielmo Marconi,” University of Bologna, since 2015, where he is currently an Associate Professor. His research interests focus on energy-efficient digital architectures. In this field, he has published more than 100 papers in international peer-reviewed conferences and journals. He is recipient of Donald O. Pederson Best Paper Award 2018, 2020 IEEE TCAS Darlington Best Paper Award, 2020 IEEE TVLSI Prize Paper Award.
\end{IEEEbiographynophoto}

\vfill
